On the complexity of generalized chromatic polynomials

J. Makowsky and B. Zilber (2004) showed that many variations of graph colorings, called CP-colorings in the sequel, give rise to graph polynomials. This is true in particular for harmonious colorings, convex colorings, mcc_t-colorings, and rainbow colorings, and many more. N. Linial (1986) showed that the chromatic polynomial $\chi(G;X)$ is #P-hard to evaluate for all but three values X=0,1,2, where evaluation is in P. This dichotomy includes evaluation at real or complex values, and has the further property that the set of points for which evaluation is in P is finite. We investigate how the complexity of evaluating univariate graph polynomials that arise from CP-colorings varies for different evaluation points. We show that for some CP-colorings (harmonious, convex) the complexity of evaluation follows a similar pattern to the chromatic polynomial. However, in other cases (proper edge colorings, mcc_t-colorings, H-free colorings) we could only obtain a dichotomy for evaluations at non-negative integer points. We also discuss some CP-colorings where we only have very partial results.

==> REV-harmonious.tex <==
%last revised 25. Dec. 2016
%\section{Harmonious colorings}

Recall that a coloring is
{\em harmonious} if it is a proper vertex coloring and
every pair of colors
occurs along some edge at most once, and $\chi_{harm}(G;X)$ is the corresponding graph polynomial.

\begin{proposition}
For every $k \in \N$ there is a polynomial time Turing machine $T(k)$ which computes
$\chi_{harm}(-;k)$. In other words $\N \subseteq \mathrm{EASY}(\chi_{harm})$ non-uniformly.
\end{proposition}
\begin{proof}
For $X=k$ a positive integer and a graph $G$ on $n$ vertices,
$\chi_{harm}(G;k) \neq 0$ implies that $G$ has  at most
$e(k)={k \choose 2 }$ 
edges.
Furthermore, there are $k^{2\cdot e(k)}$
colorings of $2 \cdot e(k)$ 
vertices with $k$ colors.
Let $i(G)$ be the number of isolated vertices of $G$,

$T(k)$ proceeds as follows:
\begin{enumerate}[(i)]
\item
Determine $|E(G)|$. If $|E(G)| \geq e(k)+1$ we have $\chi_{harm}(G;k) = 0$.
\item
Otherwise, we strip $G$ of all its isolated vertices to obtain $G'$,
which has at most $2\cdot e(k)$ vertices.  
\item
We count the colorings of $G'$ which are harmonious, i.e., $\chi_{harm}(G';k)$,
which takes time $t(k)$, 
independently of the number of vertices of $G$.
\item
Therefore $\chi_{harm}(G;k) = k^{i(G)} \cdot \chi_{harm}(G';k)$.
\end{enumerate}
It follows that $T(k)$ runs in time $O(n^2)$ where the constants depend on $k$.
\end{proof}

\begin{remark}
In spite of the low complexity of the above algorithms,
we cannot compute all the coefficients of $\chi_{harm}(G;X)$ in polynomial time.

To compute $\chi_{harm}(G;X)$ for a graph $G$ on $n$ vertices we would have to compute 
for $n+1$ values $k_1,\dots, k_{n+1}$ of $X$ 
the value of the function $\chi_{harm}(G;X)$ and then use Lagrange interpolation. However, 
the above algorithm inspects $k^{2 \cdot e(k)}$
colorings, which for at least one of the values $\chi_{harm}(G;k_i)$ is bigger than $n^{2 \cdot e(n)}$.
It follows from Theorem
\ref{th:harmonious} below that, indeed, $\chi_{harm}(G;X)$ cannot be computed in polynomial time
unless $\bP = \sharp \bP$.
\end{remark}

\begin{theorem}
\label{th:harmonious}
For each $a \in \F-\N$ the evaluation of  $\chi_{harm}(G;a)$  is $\sharp\bP$-hard.
\end{theorem}

\begin{proof}
Let $G$ be a graph. We form $S(G)$ in the following way (see Figure \ref{fig:graham}).
\\
We first form $G_1$ using $G$ by
adding a new  vertex $v_e$ for each edge $e=(u,v)$ of $G$.  Then replace the edge $e$ by two new edges
$(u,v_e)$ and $(v_e,v)$. 
\\
Using $G_1$ we now form $S(G)$:
We connect all the new vertices $v_e: e \in E(G)$ of $G_1$ 
such that they form a complete graph on $|E(G)|$ vertices.

{\bf Claim}:
For each graph $G$
\begin{gather}
\chi_{harm}(S(G);k+e(G))=\chi(G;k)\cdot\binom{k+e(G)}{e(G)}e(G)!
\label{eq:harm1}
\end{gather}
where $e(G)= |E(G)|$ and $\chi(G;k)$ is the chromatic polynomial.
\input{graham-1}

Now we look at 
\begin{gather}
\chi_{harm}(S(G \bowtie E_m); a)
\notag
\end{gather}
where $E_m$ is the edgless graph on $m$ vertices.

First we get from Equation (\ref{eq:harm1})
\begin{gather}
\chi_{harm}(S(G \bowtie E_m); a)=
\notag \\
{a \choose e(G)+m \cdot v(G)} \cdot (e(G)+m \cdot v(G))! \cdot \chi(G \bowtie E_m; a- (e(G)+m \cdot v(G))),
\label{eq:harm2}
\end{gather}
where $v(G)= |V(G)|$.

Equation (\ref{eq:harm2}) can be written as

\begin{gather}
\chi_{harm}(S(G \bowtie E_m); a)=
\notag \\
{a \choose e(G)+m \cdot v(G)} \cdot (e(G)+m \cdot v(G))! \cdot 
\notag \\
(a - e(G) - m \cdot v(G))_{(m)} \cdot
\chi(G;a-e(G)-m \cdot (v(G)+1))
\label{eq:harm3}
\end{gather}

Using Equation (\ref{eq:harm3}) several times we use Lagrange interpolation to compute
the chromatic polynomial $\chi(G;X)$. However, computing all the coefficients of $\chi(G;X)$ is $\sharp\bP$-hard.
\end{proof}
%----------------------------------------
\ifrevised
\else
Now for $k=a$ 
we have
$$\frac{\chi_{harm}(S(G);a)}{\binom{a}{e}e!}=\chi(G;a-e).$$
We have for $e=e(G)$ that
$\chi(G;a-e)$ is 
$\sharp\bP$-hard for every $a \in \F - \N$ by Theorem \ref{th:linial}.
We want to eliminate the dependence on $G$ from $a-e(G)$.

For this, we use Linial's Trick:
\\
Let $v=|V(G)|$ and $e=|E(G)|$. Then $|E(G \bowtie K_1)| = e +v$, and we get:
$$
\chi_{harm}(G \bowtie K_1;a-(e+v)+1) =  
(a-(e+v)+1) \cdot \chi_{harm}(G; a -(e+v))
$$
Which can be used for every $a \in \F-\N$.
\fi %revised
%---------------------------------
Hence we have shown:
\begin{theorem}
The Difficult Point Dichotomy DPD is true for $\chi_{harm}(G;X)$ 
\\
with 
$\mathrm{EASY}(\chi_{harm}) =\N$ non-uniformly,
\ifrevised
and $\mathrm{\sharp PHARD}(\chi_{harm}) = \F -\N$.
\else
and $\mathrm{NPHARD}(\chi_{harm}) = \F -\N$.
\fi %revised
\end{theorem}

\ifrevised
\else
In anticipation of Section \ref{se:sol} we also note that
$\chi_{harm}(G;X)$ is not $\MSOL$-definable even in the language of hypergraphs.
\fi %revised

